Stepwise functional refoundation of relational concept analysis

Relational concept analysis (RCA) is an extension of formal concept analysis allowing to deal with several related contexts simultaneously. It has been designed for learning description logic theories from data and used within various applications. A puzzling observation about RCA is that it returns a single family of concept lattices although, when the data feature circular dependencies, other solutions may be considered acceptable. The semantics of RCA, provided in an operational way, does not shed light on this issue. In this report, we define these acceptable solutions as those families of concept lattices which belong to the space determined by the initial contexts (well-formed), cannot scale new attributes (saturated), and refer only to concepts of the family (self-supported). We adopt a functional view on the RCA process by defining the space of well-formed solutions and two functions on that space: one expansive and the other contractive. We show that the acceptable solutions are the common fixed points of both functions. This is achieved step-by-step by starting from a minimal version of RCA that considers only one single context defined on a space of contexts and a space of lattices. These spaces are then joined into a single space of context-lattice pairs, which is further extended to a space of indexed families of context-lattice pairs representing the objects manippulated by RCA. We show that RCA returns the least element of the set of acceptable solutions. In addition, it is possible to build dually an operation that generates its greatest element. The set of acceptable solutions is a complete sublattice of the interval between these two elements. Its structure and how the defined functions traverse it are studied in detail.

==> dotfiles/RR-9518-dot2tex-fig1.tex <==
%%
\node (ABC) at (182.35bp,315.95bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$\empty$};
  \node (AB) at (64.347bp,182.37bp) [draw,ellipse,smconcept] {$m_2$
\nodepart{two}
$a, b$};
  \node (C) at (301.35bp,182.37bp) [draw,ellipse,smconcept] {$m_1,m_3$
\nodepart{two}
$c$};
  \node (C0) at (182.35bp,48.79bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (131.84bp,258.63bp) and (114.72bp,239.55bp)  .. (AB);
  \draw [] (ABC) ..controls (233.29bp,258.63bp) and (250.54bp,239.55bp)  .. (C);
  \draw [] (AB) ..controls (114.86bp,125.05bp) and (131.97bp,105.97bp)  .. (C0);
  \draw [] (C) ..controls (250.41bp,125.05bp) and (233.15bp,105.97bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig10.tex <==
%%
\node (DEF) at (347.27bp,449.53bp) [draw,ellipse,concept] {$\exists p.ABC$
\nodepart{two}
$\empty$};
  \node (DE) at (86.267bp,315.95bp) [draw,ellipse,concept] {$n_1, \exists p.AB$
\nodepart{two}
$\empty$};
  \node (DF) at (347.27bp,315.95bp) [draw,ellipse,concept] {$\exists p.AC$
\nodepart{two}
$\empty$};
  \node (EF) at (587.27bp,315.95bp) [draw,ellipse,concept] {$\exists p.BC$
\nodepart{two}
$\empty$};
  \node (D) at (85.267bp,182.37bp) [draw,ellipse,concept] {$\exists p.A$
\nodepart{two}
$d$};
  \node (E) at (337.27bp,182.37bp) [draw,ellipse,concept] {$n_2, \exists p.B$
\nodepart{two}
$e$};
  \node (F) at (589.27bp,182.37bp) [draw,ellipse,concept] {$\exists p.C$
\nodepart{two}
$f$};
  \node (C0) at (337.27bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (DEF) ..controls (248.38bp,398.68bp) and (192.77bp,370.64bp)  .. (DE);
  \draw [] (DEF) ..controls (347.27bp,389.05bp) and (347.27bp,376.63bp)  .. (DF);
  \draw [] (DEF) ..controls (442.67bp,396.23bp) and (495.78bp,367.11bp)  .. (EF);
  \draw [] (DE) ..controls (85.815bp,255.47bp) and (85.721bp,243.05bp)  .. (D);
  \draw [] (DE) ..controls (188.31bp,261.46bp) and (238.76bp,235.01bp)  .. (E);
  \draw [] (DF) ..controls (247.72bp,264.96bp) and (183.58bp,232.75bp)  .. (D);
  \draw [] (DF) ..controls (440.82bp,264.08bp) and (496.89bp,233.6bp)  .. (F);
  \draw [] (EF) ..controls (493.97bp,265.85bp) and (438.57bp,236.69bp)  .. (E);
  \draw [] (EF) ..controls (588.17bp,255.47bp) and (588.36bp,243.05bp)  .. (F);
  \draw [] (D) ..controls (180.92bp,131.43bp) and (241.7bp,99.689bp)  .. (C0);
  \draw [] (E) ..controls (337.27bp,121.89bp) and (337.27bp,109.47bp)  .. (C0);
  \draw [] (F) ..controls (493.62bp,131.43bp) and (432.83bp,99.689bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig11.tex <==
%%
\node (ABCD) at (64.347bp,48.79bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$a, b, c, d$};
%

==> dotfiles/RR-9518-dot2tex-fig12.tex <==
%%
\node (ABCD) at (64.347bp,48.79bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$a, b, c, d$};
%

==> dotfiles/RR-9518-dot2tex-fig13.tex <==
%%
\node (ABCD) at (77.782bp,48.79bp) [draw,ellipse,smconcept] {$\exists r.ABCD$
\nodepart{two}
$a, b, c, d$};
%

==> dotfiles/RR-9518-dot2tex-fig14.tex <==
%%
\node (ABCD) at (182.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (AB) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (CD) at (301.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.CD$
\nodepart{two}
$c, d$};
  \node (C0) at (182.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (130.39bp,257.01bp) and (114.16bp,238.91bp)  .. (AB);
  \draw [] (ABCD) ..controls (234.75bp,257.01bp) and (251.12bp,238.91bp)  .. (CD);
  \draw [] (AB) ..controls (114.86bp,125.05bp) and (131.97bp,105.97bp)  .. (C0);
  \draw [] (CD) ..controls (250.41bp,125.05bp) and (233.15bp,105.97bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig15.tex <==
%%
\node (ABCD) at (321.42bp,449.53bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (ABC) at (71.418bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABD$
\nodepart{two}
$\empty$};
  \node (ABD) at (321.42bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABC$
\nodepart{two}
$\empty$};
  \node (CD) at (564.42bp,315.95bp) [draw,ellipse,concept] {$\exists r.CD$
\nodepart{two}
$\empty$};
  \node (AB) at (80.418bp,182.37bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (C) at (317.42bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (D) at (554.42bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (317.42bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (221.63bp,396.01bp) and (167.57bp,367.56bp)  .. (ABC);
  \draw [] (ABCD) ..controls (321.42bp,389.05bp) and (321.42bp,376.63bp)  .. (ABD);
  \draw [] (ABCD) ..controls (420.06bp,395.12bp) and (473.48bp,366.2bp)  .. (CD);
  \draw [] (ABC) ..controls (75.487bp,255.47bp) and (76.336bp,243.05bp)  .. (AB);
  \draw [] (ABC) ..controls (168.63bp,262.95bp) and (224.67bp,232.98bp)  .. (C);
  \draw [] (ABD) ..controls (226.14bp,262.93bp) and (171.82bp,233.27bp)  .. (AB);
  \draw [] (ABD) ..controls (413.91bp,262.72bp) and (465.24bp,233.73bp)  .. (D);
  \draw [] (AB) ..controls (171.6bp,130.75bp) and (226.37bp,100.34bp)  .. (C0);
  \draw [] (CD) ..controls (470.44bp,264.89bp) and (411.84bp,233.67bp)  .. (C);
  \draw [] (CD) ..controls (559.9bp,255.47bp) and (558.95bp,243.05bp)  .. (D);
  \draw [] (C) ..controls (317.42bp,121.89bp) and (317.42bp,109.47bp)  .. (C0);
  \draw [] (D) ..controls (463.24bp,130.75bp) and (408.47bp,100.34bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig16.tex <==
%%
\node (AB) at (182.35bp,312.42bp) [draw,ellipse,concept] {$\exists p.CD$
            \nodepart{two}
            $\empty$};
  \node (A) at (64.347bp,180.25bp) [draw,ellipse,concept] {$\exists p.C$
            \nodepart{two}
            $a$};
  \node (B) at (301.35bp,180.25bp) [draw,ellipse,concept] {$\exists p.D$
            \nodepart{two}
            $b$};
  \node (C0) at (182.35bp,48.083bp) [draw,ellipse,concept] {$\empty$
            \nodepart{two}
            $\empty$};
  \draw [] (AB) ..controls (130.56bp,254.29bp) and (114.1bp,236.13bp)  .. (A);
  \draw [] (AB) ..controls (234.57bp,254.29bp) and (251.17bp,236.13bp)  .. (B);
  \draw [] (A) ..controls (114.18bp,124.28bp) and (130.4bp,106.38bp)  .. (C0);
  \draw [] (B) ..controls (251.27bp,124.47bp) and (234.67bp,106.32bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig17.tex <==
%%
\node (CD) at (182.35bp,315.95bp) [draw,ellipse,concept] {$\exists q.AB$
\nodepart{two}
$\empty$};
  \node (C) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\exists q.A$
\nodepart{two}
$c$};
  \node (D) at (301.35bp,182.37bp) [draw,ellipse,concept] {$\exists q.B$
\nodepart{two}
$d$};
  \node (C0) at (182.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (CD) ..controls (131.66bp,258.43bp) and (114.79bp,239.62bp)  .. (C);
  \draw [] (CD) ..controls (233.46bp,258.43bp) and (250.48bp,239.62bp)  .. (D);
  \draw [] (C) ..controls (114.86bp,125.05bp) and (131.97bp,105.97bp)  .. (C0);
  \draw [] (D) ..controls (250.41bp,125.05bp) and (233.15bp,105.97bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig18.tex <==
%%
\node (AB) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists p.CD$
\nodepart{two}
$b$};
  \node (A) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists p.C$
\nodepart{two}
$a$};
  \draw [] (AB) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (A);
%

==> dotfiles/RR-9518-dot2tex-fig19.tex <==
%%
\node (CD) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists q.AB$
\nodepart{two}
$d$};
  \node (C) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists q.A$
\nodepart{two}
$c$};
  \draw [] (CD) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (C);
%

==> dotfiles/RR-9518-dot2tex-fig2.tex <==
%%
\node (ABC) at (182.35bp,315.95bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$\empty$};
  \node (AB) at (64.347bp,182.37bp) [draw,ellipse,smconcept] {$m_2$
\nodepart{two}
$a, b$};
  \node (C) at (301.35bp,182.37bp) [draw,ellipse,smconcept] {$m_1,m_3$
\nodepart{two}
$c$};
  \node (C0) at (182.35bp,48.79bp) [draw,ellipse,smconcept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (131.84bp,258.63bp) and (114.72bp,239.55bp)  .. (AB);
  \draw [] (ABC) ..controls (233.29bp,258.63bp) and (250.54bp,239.55bp)  .. (C);
  \draw [] (AB) ..controls (114.86bp,125.05bp) and (131.97bp,105.97bp)  .. (C0);
  \draw [] (C) ..controls (250.41bp,125.05bp) and (233.15bp,105.97bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig20.tex <==
%%
\node (AB) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists p.CD$
\nodepart{two}
$a$};
  \node (B) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists p.D$
\nodepart{two}
$b$};
  \draw [] (AB) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (B);
%

==> dotfiles/RR-9518-dot2tex-fig21.tex <==
%%
\node (CD) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists q.AB$
\nodepart{two}
$c$};
  \node (D) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists q.B$
\nodepart{two}
$d$};
  \draw [] (CD) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (D);
%

==> dotfiles/RR-9518-dot2tex-fig22.tex <==
%%
\node (AB) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists p.CD$
\nodepart{two}
$b$};
  \node (A) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists p.C$
\nodepart{two}
$a$};
  \draw [] (AB) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (A);
%

==> dotfiles/RR-9518-dot2tex-fig23.tex <==
%%
\node (CD) at (66.468bp,182.37bp) [draw,ellipse,concept] {$\exists q.AB$
\nodepart{two}
$c$};
  \node (D) at (66.468bp,48.79bp) [draw,ellipse,concept] {$\exists q.B$
\nodepart{two}
$d$};
  \draw [] (CD) ..controls (66.468bp,121.89bp) and (66.468bp,109.47bp)  .. (D);
%

==> dotfiles/RR-9518-dot2tex-fig24.tex <==
%%
\node (ABCD) at (244.36bp,449.53bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \node (ABC) at (127.36bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABD$
\nodepart{two}
$c$};
  \node (D) at (383.36bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (AB) at (105.36bp,182.37bp) [draw,ellipse,concept] {$\exists r.B, \exists r.AB$
\nodepart{two}
$a, b$};
  \node (C0) at (244.36bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (194.68bp,392.66bp) and (178.24bp,374.18bp)  .. (ABC);
  \draw [] (ABCD) ..controls (293.39bp,355.0bp) and (334.19bp,277.16bp)  .. (D);
  \draw [] (ABC) ..controls (117.45bp,255.67bp) and (115.34bp,243.04bp)  .. (AB);
  \draw [] (D) ..controls (324.92bp,126.05bp) and (302.81bp,105.12bp)  .. (C0);
  \draw [] (AB) ..controls (168.13bp,121.95bp) and (187.64bp,103.48bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig25.tex <==
%%
\node (ABCD) at (651.73bp,449.53bp) [draw,ellipse,concept] {$\exists r.ACD$,$\exists r.BCD$,$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (ABC) at (181.73bp,315.95bp) [draw,ellipse,concept] {$\exists r.AD$,$\exists r.BD$,$\exists r.ABD$
\nodepart{two}
$\empty$};
  \node (ABD) at (651.73bp,315.95bp) [draw,ellipse,concept] {$\exists r.AC$,$\exists r.BC$,$\exists r.ABC$
\nodepart{two}
$\empty$};
  \node (CD) at (1004.7bp,315.95bp) [draw,ellipse,concept] {$\exists r.CD$
\nodepart{two}
$\empty$};
  \node (AB) at (307.73bp,182.37bp) [draw,ellipse,concept] {$\exists r.A$,$\exists r.B$,$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (C) at (641.73bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (D) at (878.73bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (641.73bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (454.53bp,393.33bp) and (372.38bp,370.33bp)  .. (ABC);
  \draw [] (ABCD) ..controls (651.73bp,389.05bp) and (651.73bp,376.63bp)  .. (ABD);
  \draw [] (ABCD) ..controls (803.08bp,395.39bp) and (846.39bp,379.68bp)  .. (885.73bp,364.74bp) .. controls (906.33bp,356.92bp) and (928.8bp,348.0bp)  .. (CD);
  \draw [] (ABC) ..controls (238.34bp,255.84bp) and (251.54bp,242.05bp)  .. (AB);
  \draw [] (ABC) ..controls (384.67bp,270.65bp) and (457.88bp,252.04bp)  .. (522.73bp,231.16bp) .. controls (543.81bp,224.37bp) and (566.49bp,215.64bp)  .. (C);
  \draw [] (ABD) ..controls (503.84bp,258.39bp) and (451.06bp,238.2bp)  .. (AB);
  \draw [] (ABD) ..controls (760.0bp,252.19bp) and (798.35bp,229.96bp)  .. (D);
  \draw [] (AB) ..controls (463.33bp,120.07bp) and (535.89bp,91.486bp)  .. (C0);
  \draw [] (CD) ..controls (929.32bp,283.19bp) and (906.68bp,274.36bp)  .. (885.73bp,267.16bp) .. controls (831.05bp,248.36bp) and (815.4bp,249.96bp)  .. (760.73bp,231.16bp) .. controls (739.78bp,223.96bp) and (717.14bp,215.14bp)  .. (C);
  \draw [] (CD) ..controls (951.16bp,259.01bp) and (932.38bp,239.4bp)  .. (D);
  \draw [] (C) ..controls (641.73bp,121.89bp) and (641.73bp,109.47bp)  .. (C0);
  \draw [] (D) ..controls (787.55bp,130.75bp) and (732.78bp,100.34bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig26.tex <==
%%
\node (ABCD) at (321.42bp,449.53bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (ABC) at (71.418bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABD$
\nodepart{two}
$\empty$};
  \node (ABD) at (321.42bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABC$
\nodepart{two}
$\empty$};
  \node (CD) at (564.42bp,315.95bp) [draw,ellipse,concept] {$\exists r.CD$
\nodepart{two}
$\empty$};
  \node (AB) at (80.418bp,182.37bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (C) at (317.42bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (D) at (554.42bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (317.42bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (221.63bp,396.01bp) and (167.57bp,367.56bp)  .. (ABC);
  \draw [] (ABCD) ..controls (321.42bp,389.05bp) and (321.42bp,376.63bp)  .. (ABD);
  \draw [] (ABCD) ..controls (420.06bp,395.12bp) and (473.48bp,366.2bp)  .. (CD);
  \draw [] (ABC) ..controls (75.487bp,255.47bp) and (76.336bp,243.05bp)  .. (AB);
  \draw [] (ABC) ..controls (168.63bp,262.95bp) and (224.67bp,232.98bp)  .. (C);
  \draw [] (ABD) ..controls (226.14bp,262.93bp) and (171.82bp,233.27bp)  .. (AB);
  \draw [] (ABD) ..controls (413.91bp,262.72bp) and (465.24bp,233.73bp)  .. (D);
  \draw [] (AB) ..controls (171.6bp,130.75bp) and (226.37bp,100.34bp)  .. (C0);
  \draw [] (CD) ..controls (470.44bp,264.89bp) and (411.84bp,233.67bp)  .. (C);
  \draw [] (CD) ..controls (559.9bp,255.47bp) and (558.95bp,243.05bp)  .. (D);
  \draw [] (C) ..controls (317.42bp,121.89bp) and (317.42bp,109.47bp)  .. (C0);
  \draw [] (D) ..controls (463.24bp,130.75bp) and (408.47bp,100.34bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig27.tex <==
%%
\node (ABC) at (368.36bp,315.95bp) [draw,ellipse,concept] {$\exists p.DEF, \exists p.DF, \exists p.EF$
\nodepart{two}
$\empty$};
  \node (AB) at (175.36bp,182.37bp) [draw,ellipse,concept] {$m_2, \exists p.D, \exists p.E, \exists p.DE$
\nodepart{two}
$a$, $b$};
  \node (C) at (562.36bp,182.37bp) [draw,ellipse,concept] {$m_1, m_3, \exists p.F$
\nodepart{two}
$c$};
  \node (C0) at (368.36bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (283.3bp,256.96bp) and (260.94bp,241.72bp)  .. (AB);
  \draw [] (ABC) ..controls (456.14bp,255.41bp) and (481.75bp,238.05bp)  .. (C);
  \draw [] (AB) ..controls (266.81bp,119.03bp) and (296.7bp,98.649bp)  .. (C0);
  \draw [] (C) ..controls (475.92bp,122.74bp) and (442.43bp,100.03bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig28.tex <==
%%
\node (DEF) at (347.27bp,449.53bp) [draw,ellipse,concept] {$\exists p.ABC$
\nodepart{two}
$\empty$};
  \node (DE) at (86.267bp,315.95bp) [draw,ellipse,concept] {$n_1, \exists p.AB$
\nodepart{two}
$\empty$};
  \node (DF) at (347.27bp,315.95bp) [draw,ellipse,concept] {$\exists p.AC$
\nodepart{two}
$\empty$};
  \node (EF) at (587.27bp,315.95bp) [draw,ellipse,concept] {$\exists p.BC$
\nodepart{two}
$\empty$};
  \node (D) at (85.267bp,182.37bp) [draw,ellipse,concept] {$\exists p.A$
\nodepart{two}
$d$};
  \node (E) at (337.27bp,182.37bp) [draw,ellipse,concept] {$n_2, \exists p.B$
\nodepart{two}
$e$};
  \node (F) at (589.27bp,182.37bp) [draw,ellipse,concept] {$\exists p.C$
\nodepart{two}
$f$};
  \node (C0) at (337.27bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (DEF) ..controls (248.38bp,398.68bp) and (192.77bp,370.64bp)  .. (DE);
  \draw [] (DEF) ..controls (347.27bp,389.05bp) and (347.27bp,376.63bp)  .. (DF);
  \draw [] (DEF) ..controls (442.67bp,396.23bp) and (495.78bp,367.11bp)  .. (EF);
  \draw [] (DE) ..controls (85.815bp,255.47bp) and (85.721bp,243.05bp)  .. (D);
  \draw [] (DE) ..controls (188.31bp,261.46bp) and (238.76bp,235.01bp)  .. (E);
  \draw [] (DF) ..controls (247.72bp,264.96bp) and (183.58bp,232.75bp)  .. (D);
  \draw [] (DF) ..controls (440.82bp,264.08bp) and (496.89bp,233.6bp)  .. (F);
  \draw [] (EF) ..controls (493.97bp,265.85bp) and (438.57bp,236.69bp)  .. (E);
  \draw [] (EF) ..controls (588.17bp,255.47bp) and (588.36bp,243.05bp)  .. (F);
  \draw [] (D) ..controls (180.92bp,131.43bp) and (241.7bp,99.689bp)  .. (C0);
  \draw [] (E) ..controls (337.27bp,121.89bp) and (337.27bp,109.47bp)  .. (C0);
  \draw [] (F) ..controls (493.62bp,131.43bp) and (432.83bp,99.689bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig29.tex <==
%%
\node (DEF) at (210.27bp,449.53bp) [draw,ellipse,concept] {$\exists p.ABC$
\nodepart{two}
$\empty$};
  \node (DE) at (86.267bp,315.95bp) [draw,ellipse,concept] {$n_1, \exists p.AB$
\nodepart{two}
$d$};
  \node (F) at (332.27bp,182.37bp) [draw,ellipse,concept] {$\exists q.C$
\nodepart{two}
$f$};
  \node (E) at (92.267bp,182.37bp) [draw,ellipse,concept] {$n_2$
\nodepart{two}
$e$};
  \node (C0) at (210.27bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (DEF) ..controls (157.53bp,392.58bp) and (140.97bp,375.0bp)  .. (DE);
  \draw [] (DEF) ..controls (253.82bp,353.88bp) and (289.08bp,277.25bp)  .. (F);
  \draw [] (DE) ..controls (88.98bp,255.47bp) and (89.546bp,243.05bp)  .. (E);
  \draw [] (E) ..controls (142.78bp,125.05bp) and (159.89bp,105.97bp)  .. (C0);
  \draw [] (F) ..controls (280.22bp,125.24bp) and (262.28bp,105.89bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig3.tex <==
%%
\node (ABC) at (182.35bp,315.95bp) [draw,ellipse,concept] {$$
\nodepart{two}
$\empty$};
  \node (AB) at (64.347bp,182.37bp) [draw,ellipse,concept] {$m_2$
\nodepart{two}
$a, b$};
  \node (C) at (301.35bp,182.37bp) [draw,ellipse,concept] {$m_1, m_3$
\nodepart{two}
$c$};
  \node (C0) at (182.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (131.84bp,258.63bp) and (114.72bp,239.55bp)  .. (AB);
  \draw [] (ABC) ..controls (233.29bp,258.63bp) and (250.54bp,239.55bp)  .. (C);
  \draw [] (AB) ..controls (114.86bp,125.05bp) and (131.97bp,105.97bp)  .. (C0);
  \draw [] (C) ..controls (250.41bp,125.05bp) and (233.15bp,105.97bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig30.tex <==
%%
\node (ABC) at (302.52bp,315.95bp) [draw,ellipse,concept] {$\exists p.DEF$
\nodepart{two}
$\empty$};
  \node (AB) at (131.52bp,182.37bp) [draw,ellipse,concept] {$m_2, \exists p.E, \exists p.DE$
\nodepart{two}
$a$, $b$};
  \node (C) at (474.52bp,182.37bp) [draw,ellipse,concept] {$m_1, m_3, \exists p.F$
\nodepart{two}
$c$};
  \node (C0) at (302.52bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (234.73bp,262.79bp) and (209.69bp,243.52bp)  .. (AB);
  \draw [] (ABC) ..controls (371.6bp,262.1bp) and (398.04bp,241.88bp)  .. (C);
  \draw [] (AB) ..controls (210.65bp,120.48bp) and (236.41bp,100.66bp)  .. (C0);
  \draw [] (C) ..controls (397.38bp,122.35bp) and (369.85bp,101.3bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig31.tex <==
%%
\node (ABCD) at (342.35bp,449.53bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (ABC) at (217.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABD$
\nodepart{two}
$\empty$};
  \node (ABD) at (467.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABC$
\nodepart{two}
$\empty$};
  \node (AB) at (342.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.B, \exists r.AB$
\nodepart{two}
$a, b$};
  \node (C) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (D) at (620.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (342.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (287.96bp,391.28bp) and (270.64bp,373.05bp)  .. (ABC);
  \draw [] (ABCD) ..controls (396.73bp,391.28bp) and (414.05bp,373.05bp)  .. (ABD);
  \draw [] (ABC) ..controls (270.07bp,259.45bp) and (286.22bp,242.45bp)  .. (AB);
  \draw [] (ABC) ..controls (152.4bp,259.1bp) and (127.21bp,237.44bp)  .. (C);
  \draw [] (ABD) ..controls (532.29bp,259.1bp) and (557.48bp,237.44bp)  .. (D);
  \draw [] (ABD) ..controls (414.95bp,259.79bp) and (398.74bp,242.74bp)  .. (AB);
  \draw [] (D) ..controls (517.1bp,132.5bp) and (445.41bp,98.573bp)  .. (C0);
  \draw [] (AB) ..controls (342.35bp,121.89bp) and (342.35bp,109.47bp)  .. (C0);
  \draw [] (C) ..controls (167.59bp,132.5bp) and (239.28bp,98.573bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig32.tex <==
%%
\node (ABCD) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$c, d$};
  \node (AB) at (64.347bp,48.79bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \draw [] (ABCD) ..controls (64.347bp,121.89bp) and (64.347bp,109.47bp)  .. (AB);
%

==> dotfiles/RR-9518-dot2tex-fig33.tex <==
%%
\node (ABCD) at (301.35bp,449.53bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (ABC) at (176.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABD$
\nodepart{two}
$\empty$};
  \node (ABD) at (426.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABC$
\nodepart{two}
$\empty$};
  \node (AB) at (301.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (C) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (D) at (538.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (301.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (246.96bp,391.28bp) and (229.64bp,373.05bp)  .. (ABC);
  \draw [] (ABCD) ..controls (355.73bp,391.28bp) and (373.05bp,373.05bp)  .. (ABD);
  \draw [] (ABC) ..controls (230.51bp,257.94bp) and (248.51bp,238.99bp)  .. (AB);
  \draw [] (ABC) ..controls (127.45bp,257.51bp) and (112.15bp,239.53bp)  .. (C);
  \draw [] (ABD) ..controls (475.24bp,257.51bp) and (490.54bp,239.53bp)  .. (D);
  \draw [] (ABD) ..controls (372.37bp,258.13bp) and (354.12bp,238.92bp)  .. (AB);
  \draw [] (D) ..controls (447.17bp,130.75bp) and (392.4bp,100.34bp)  .. (C0);
  \draw [] (AB) ..controls (301.35bp,121.89bp) and (301.35bp,109.47bp)  .. (C0);
  \draw [] (C) ..controls (155.53bp,130.75bp) and (210.29bp,100.34bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig34.tex <==
%%
\node (ABCD) at (77.782bp,182.37bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$c, d$};
  \node (AB) at (77.782bp,48.79bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \draw [] (ABCD) ..controls (77.782bp,121.89bp) and (77.782bp,109.47bp)  .. (AB);
%

==> dotfiles/RR-9518-dot2tex-fig35.tex <==
%%
\node (ABCD) at (301.35bp,315.95bp) [draw,ellipse,concept] {$\exists r.ABCD$
\nodepart{two}
$\empty$};
  \node (C) at (64.347bp,182.37bp) [draw,ellipse,concept] {$\exists r.D$
\nodepart{two}
$c$};
  \node (AB) at (301.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.AB$
\nodepart{two}
$a, b$};
  \node (D) at (538.35bp,182.37bp) [draw,ellipse,concept] {$\exists r.C$
\nodepart{two}
$d$};
  \node (C0) at (301.35bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABCD) ..controls (204.62bp,261.25bp) and (153.48bp,232.86bp)  .. (C);
  \draw [] (ABCD) ..controls (301.35bp,255.47bp) and (301.35bp,243.05bp)  .. (AB);
  \draw [] (ABCD) ..controls (398.07bp,261.25bp) and (449.21bp,232.86bp)  .. (D);
  \draw [] (C) ..controls (155.53bp,130.75bp) and (210.29bp,100.34bp)  .. (C0);
  \draw [] (AB) ..controls (301.35bp,121.89bp) and (301.35bp,109.47bp)  .. (C0);
  \draw [] (D) ..controls (447.17bp,130.75bp) and (392.4bp,100.34bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig4.tex <==
%%
\node (DEF) at (64.347bp,315.95bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$f$};
  \node (DE) at (64.347bp,182.37bp) [draw,ellipse,concept] {$n_1$
\nodepart{two}
$d$};
  \node (E) at (64.347bp,48.79bp) [draw,ellipse,concept] {$n_2$
\nodepart{two}
$e$};
  \draw [] (DEF) ..controls (64.347bp,255.47bp) and (64.347bp,243.05bp)  .. (DE);
  \draw [] (DE) ..controls (64.347bp,121.89bp) and (64.347bp,109.47bp)  .. (E);
%

==> dotfiles/RR-9518-dot2tex-fig5.tex <==
%%
\node (ABC) at (224.46bp,449.53bp) [draw,ellipse,concept] {$\exists p.DEF$
\nodepart{two}
$\empty$};
  \node (AB) at (95.459bp,315.95bp) [draw,ellipse,concept] {$m_2$,$\exists p.DE$
\nodepart{two}
$a$};
  \node (C) at (347.46bp,182.37bp) [draw,ellipse,concept] {$m_1, m_3$
\nodepart{two}
$c$};
  \node (B) at (105.46bp,182.37bp) [draw,ellipse,concept] {$\exists p.E$
\nodepart{two}
$b$};
  \node (C0) at (223.46bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (170.09bp,393.07bp) and (152.98bp,375.63bp)  .. (AB);
  \draw [] (ABC) ..controls (268.37bp,353.88bp) and (303.91bp,277.25bp)  .. (C);
  \draw [] (AB) ..controls (99.98bp,255.47bp) and (100.92bp,243.05bp)  .. (B);
  \draw [] (B) ..controls (155.97bp,125.05bp) and (173.08bp,105.97bp)  .. (C0);
  \draw [] (C) ..controls (294.74bp,125.43bp) and (276.26bp,105.82bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig6.tex <==
%%
\node (DEF) at (210.27bp,449.53bp) [draw,ellipse,concept] {$\exists q.ABC$
\nodepart{two}
$\empty$};
  \node (DE) at (86.267bp,315.95bp) [draw,ellipse,concept] {$n_1, \exists q.AB$
\nodepart{two}
$d$};
  \node (F) at (332.27bp,182.37bp) [draw,ellipse,concept] {$\exists q.C$
\nodepart{two}
$f$};
  \node (E) at (92.267bp,182.37bp) [draw,ellipse,concept] {$n_2$
\nodepart{two}
$e$};
  \node (C0) at (210.27bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (DEF) ..controls (157.53bp,392.58bp) and (140.97bp,375.0bp)  .. (DE);
  \draw [] (DEF) ..controls (253.82bp,353.88bp) and (289.08bp,277.25bp)  .. (F);
  \draw [] (DE) ..controls (88.98bp,255.47bp) and (89.546bp,243.05bp)  .. (E);
  \draw [] (E) ..controls (142.78bp,125.05bp) and (159.89bp,105.97bp)  .. (C0);
  \draw [] (F) ..controls (280.22bp,125.24bp) and (262.28bp,105.89bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig7.tex <==
%%
\node (ABC) at (213.39bp,470.75bp) [draw,ellipse,concept] {$\exists p.DEF$
\nodepart{two}
$\empty$};
  \node (AB) at (88.388bp,337.17bp) [draw,ellipse,concept] {$m_2, \exists p.DE$
\nodepart{two}
$a$};
  \node (C) at (336.39bp,192.98bp) [draw,ellipse,concept] {$m_1, m_3$,\\$\exists p.F$
\nodepart{two}
$c$};
  \node (B) at (92.388bp,192.98bp) [draw,ellipse,concept] {$\exists p.E$
\nodepart{two}
$b$};
  \node (C0) at (213.39bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (160.23bp,413.79bp) and (143.53bp,396.21bp)  .. (AB);
  \draw [] (ABC) ..controls (255.29bp,375.81bp) and (289.0bp,300.23bp)  .. (C);
  \draw [] (AB) ..controls (90.16bp,273.2bp) and (90.619bp,256.89bp)  .. (B);
  \draw [] (B) ..controls (143.09bp,132.4bp) and (162.59bp,109.48bp)  .. (C0);
  \draw [] (C) ..controls (280.2bp,127.02bp) and (263.06bp,107.21bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig8.tex <==
%%
\node (DEF) at (210.27bp,449.53bp) [draw,ellipse,concept] {$\exists q.ABC$
\nodepart{two}
$\empty$};
  \node (DE) at (86.267bp,315.95bp) [draw,ellipse,concept] {$n_1, \exists q.AB$
\nodepart{two}
$d$};
  \node (F) at (337.27bp,182.37bp) [draw,ellipse,concept] {$\exists q.C$
\nodepart{two}
$f$};
  \node (E) at (85.267bp,182.37bp) [draw,ellipse,concept] {$n_2, \exists q.B$
\nodepart{two}
$e$};
  \node (C0) at (211.27bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (DEF) ..controls (157.53bp,392.58bp) and (140.97bp,375.0bp)  .. (DE);
  \draw [] (DEF) ..controls (255.5bp,354.09bp) and (292.43bp,276.99bp)  .. (F);
  \draw [] (DE) ..controls (85.815bp,255.47bp) and (85.721bp,243.05bp)  .. (E);
  \draw [] (E) ..controls (140.71bp,123.48bp) and (158.47bp,104.93bp)  .. (C0);
  \draw [] (F) ..controls (283.7bp,125.43bp) and (264.92bp,105.82bp)  .. (C0);
%

==> dotfiles/RR-9518-dot2tex-fig9.tex <==
%%
\node (ABC) at (349.39bp,449.53bp) [draw,ellipse,concept] {$\exists p.DEF$
\nodepart{two}
$\empty$};
  \node (AB) at (88.388bp,315.95bp) [draw,ellipse,concept] {$m_2, \exists p.DE$
\nodepart{two}
$\empty$};
  \node (AC) at (349.39bp,315.95bp) [draw,ellipse,concept] {$\exists p.DF$
\nodepart{two}
$\empty$};
  \node (BC) at (586.39bp,315.95bp) [draw,ellipse,concept] {$\exists p.EF$
\nodepart{two}
$\empty$};
  \node (A) at (81.388bp,182.37bp) [draw,ellipse,concept] {$\exists p.D$
\nodepart{two}
$a$};
  \node (B) at (318.39bp,182.37bp) [draw,ellipse,concept] {$\exists p.E$
\nodepart{two}
$b$};
  \node (C) at (594.39bp,182.37bp) [draw,ellipse,concept] {$m_1, m_3, \exists p.F$
\nodepart{two}
$c$};
  \node (C0) at (318.39bp,48.79bp) [draw,ellipse,concept] {$\empty$
\nodepart{two}
$\empty$};
  \draw [] (ABC) ..controls (251.34bp,399.1bp) and (195.79bp,371.1bp)  .. (AB);
  \draw [] (ABC) ..controls (349.39bp,389.05bp) and (349.39bp,376.63bp)  .. (AC);
  \draw [] (ABC) ..controls (443.74bp,396.15bp) and (496.41bp,366.91bp)  .. (BC);
  \draw [] (AB) ..controls (85.224bp,255.47bp) and (84.563bp,243.05bp)  .. (A);
  \draw [] (AB) ..controls (185.99bp,259.12bp) and (232.51bp,232.5bp)  .. (B);
  \draw [] (AC) ..controls (248.86bp,265.59bp) and (181.81bp,232.67bp)  .. (A);
  \draw [] (AC) ..controls (438.19bp,267.26bp) and (487.32bp,240.87bp)  .. (C);
  \draw [] (BC) ..controls (486.06bp,265.69bp) and (418.6bp,232.57bp)  .. (B);
  \draw [] (BC) ..controls (590.01bp,255.47bp) and (590.76bp,243.05bp)  .. (C);
  \draw [] (A) ..controls (172.57bp,130.75bp) and (227.34bp,100.34bp)  .. (C0);
  \draw [] (B) ..controls (318.39bp,121.89bp) and (318.39bp,109.47bp)  .. (C0);
  \draw [] (C) ..controls (475.44bp,124.66bp) and (415.44bp,96.06bp)  .. (C0);
%
